Minimax-Optimal Off-Policy Evaluation with Linear Function Approximation

This paper studies the statistical theory of batch data reinforcement learning with function approximation. Consider the off-policy evaluation problem, which is to estimate the cumulative value of a new target policy from logged history generated by unknown behavioral policies. We study a regression-based fitted Q iteration method, and show that it is equivalent to a model-based method that estimates a conditional mean embedding of the transition operator. We prove that this method is information-theoretically optimal and has nearly minimal estimation error. In particular, by leveraging contraction property of Markov processes and martingale concentration, we establish a finite-sample instance-dependent error upper bound and a nearly-matching minimax lower bound. The policy evaluation error depends sharply on a restricted $\chi^2$-divergence over the function class between the long-term distribution of the target policy and the distribution of past data. This restricted $\chi^2$-divergence is both instance-dependent and function-class-dependent. It characterizes the statistical limit of off-policy evaluation. Further, we provide an easily computable confidence bound for the policy evaluator, which may be useful for optimistic planning and safe policy improvement.

==> 06-discussion.tex <==
When upper and lower bounds match

\begin{itemize}
	\item If we have $\phi(s,a)^{\top} \Sigma^{-1} \phi(s',a') \geq 0$ for any $(s,a), (s', a') \in \mathcal{X}$, then the first-order term in upper bound matches the rate of minimax lower bound.
	\item Block diagonal \\
	time-dependent state $(s,h)$
\end{itemize}

Our proposed estimator $\widehat{v}^{\pi}$ contains powers of matrix $\widehat{M}^{\pi}$ in its definition. Since the error in $\widehat{M}^{\pi}$ accumulates multiplicatively in the powers, it may result in an exponentially high error. This problem is called the ``curse of horizon''. Fortunately, according to our analysis in Theorem \ref{UpperBound},   does not deteriorate sample complexity. 

mismatch - chi-square divergence

results in the special tabular case
